Deep-URL: A Model-Aware Approach To Blind Deconvolution Based On Deep Unfolded Richardson-Lucy Network

The lack of interpretability in current deep learning models causes serious concerns as they are extensively used for various life-critical applications. Hence, it is of paramount importance to develop interpretable deep learning models. In this paper, we consider the problem of blind deconvolution and propose a novel model-aware deep architecture that allows for the recovery of both the blur kernel and the sharp image from the blurred image. In particular, we propose the Deep Unfolded Richardson-Lucy (Deep-URL) framework -- an interpretable deep-learning architecture that can be seen as an amalgamation of classical estimation technique and deep neural network, and consequently leads to improved performance. Our numerical investigations demonstrate significant improvement compared to state-of-the-art algorithms.

==> ICIP'2020/symbols.tex <==
%% Short symbol commands for LaTex
\usepackage{amsmath}
\usepackage{algpseudocode}
\usepackage{amsthm}
\usepackage{dsfont}
\usepackage{algorithm}
\usepackage{thmtools}
\usepackage{amssymb}
\usepackage[dvipsnames]{xcolor}

\def \Author{Arindam~Bose}
\def \Version{2.0.11}
\def \Update{\today}

% Lower case bold English alphabets
\def\ba{\boldsymbol{a}}
\def\bb{\boldsymbol{b}}
\def\bc{\boldsymbol{c}}
\def\bd{\boldsymbol{d}}
\def\be{\boldsymbol{e}}
\def\bdf{\boldsymbol{f}}
\def\bg{\boldsymbol{g}}
\def\bh{\boldsymbol{h}}
\def\bi{\boldsymbol{i}}
\def\bj{\boldsymbol{j}}
\def\bk{\boldsymbol{k}}
\def\bl{\boldsymbol{l}}
\def\bm{\boldsymbol{m}}
\def\bn{\boldsymbol{n}}
\def\bo{\boldsymbol{o}}
\def\bp{\boldsymbol{p}}
\def\bq{\boldsymbol{q}}
\def\br{\boldsymbol{r}}
\def\bs{\boldsymbol{s}}
\def\bt{\boldsymbol{t}}
\def\bu{\boldsymbol{u}}
\def\bv{\boldsymbol{v}}
\def\bw{\boldsymbol{w}}
\def\bx{\boldsymbol{x}}
\def\by{\boldsymbol{y}}
\def\bz{\boldsymbol{z}}

% Upper case bold English alphabets
\def\bA{\boldsymbol{A}}
\def\bB{\boldsymbol{B}}
\def\bC{\boldsymbol{C}}
\def\bD{\boldsymbol{D}}
\def\bE{\boldsymbol{E}}
\def\bF{\boldsymbol{F}}
\def\bG{\boldsymbol{G}}
\def\bH{\boldsymbol{H}}
\def\bI{\boldsymbol{I}}
\def\bJ{\boldsymbol{J}}
\def\bK{\boldsymbol{K}}
\def\bL{\boldsymbol{L}}
\def\bN{\boldsymbol{N}}
\def\bM{\boldsymbol{M}}
\def\bO{\boldsymbol{O}}
\def\bP{\boldsymbol{P}}
\def\bQ{\boldsymbol{Q}}
\def\bR{\boldsymbol{R}}
\def\bS{\boldsymbol{S}}
\def\bT{\boldsymbol{T}}
\def\bU{\boldsymbol{U}}
\def\bV{\boldsymbol{V}}
\def\bW{\boldsymbol{W}}
\def\bX{\boldsymbol{X}}
\def\bY{\boldsymbol{Y}}
\def\bZ{\boldsymbol{Z}}

% Bold Greek alphabets
\def\balpha{\boldsymbol{\alpha}}
\def\bbeta{\boldsymbol{\beta}}
\def\bgamma{\boldsymbol{\gamma}}
\def\bGamma{\boldsymbol{\Gamma}}
\def\bdelta{\boldsymbol{\delta}}
\def\bDelta{\boldsymbol{\Delta}}
\def\bepsilon{\boldsymbol{\epsilon}}
\def\bvarepsilon{\boldsymbol{\varepsilon}}
\def\bzeta{\boldsymbol{\zeta}}
\def\bdeta{\boldsymbol{\eta}}
\def\btheta{\boldsymbol{\theta}}
\def\bvartheta{\boldsymbol{\vartheta}}
\def\bTheta{\boldsymbol{\Theta}}
\def\biota{\boldsymbol{\iota}}
\def\bkappa{\boldsymbol{\kappa}}
\def\blambda{\boldsymbol{\lambda}}
\def\bLambda{\boldsymbol{\Lambda}}
\def\bmu{\boldsymbol{\mu}}
\def\bnu{\boldsymbol{\nu}}
\def\bxi{\boldsymbol{\xi}}
\def\bXi{\boldsymbol{\Xi}}
\def\bpi{\boldsymbol{\pi}}
\def\bPi{\boldsymbol{\Pi}}
\def\brho{\boldsymbol{\rho}}
\def\bvarrho{\boldsymbol{\varrho}}
\def\bsigma{\boldsymbol{\sigma}}
\def\bSigma{\boldsymbol{\Sigma}}
\def\btau{\boldsymbol{\tau}}
\def\bupsilon{\boldsymbol{\upsilon}}
\def\bUpsilon{\boldsymbol{\Upsilon}}
\def\bphi{\boldsymbol{\phi}}
\def\bvarphi{\boldsymbol{\varphi}}
\def\bPhi{\boldsymbol{\Phi}}
\def\bchi{\boldsymbol{\chi}}
\def\bpsi{\boldsymbol{\psi}}
\def\bPsi{\boldsymbol{\Psi}}
\def\bomega{\boldsymbol{\omega}}
\def\bOmega{\boldsymbol{\Omega}}

% Mathbf lower case English alphabets
\def\mba{\mathbf{a}}
\def\mbb{\mathbf{b}}
\def\mbc{\mathbf{c}}
\def\mbd{\mathbf{d}}
\def\mbe{\mathbf{e}}
\def\mbf{\mathbf{f}}
\def\mbg{\mathbf{g}}
\def\mbh{\mathbf{h}}
\def\mbi{\mathbf{i}}
\def\mbj{\mathbf{j}}
\def\mbk{\mathbf{k}}
\def\mbl{\mathbf{l}}
\def\mbm{\mathbf{m}}
\def\mbn{\mathbf{n}}
\def\mbo{\mathbf{o}}
\def\mbp{\mathbf{p}}
\def\mbq{\mathbf{q}}
\def\mbr{\mathbf{r}}
\def\mbs{\mathbf{s}}
\def\mbt{\mathbf{t}}
\def\mbu{\mathbf{u}}
\def\mbv{\mathbf{v}}
\def\mbw{\mathbf{w}}
\def\mbx{\mathbf{x}}
\def\mby{\mathbf{y}}
\def\mbz{\mathbf{z}}

% Mathbf upper case English alphabets
\def\mbA{\mathbf{A}}
\def\mbB{\mathbf{B}}
\def\mbC{\mathbf{C}}
\def\mbD{\mathbf{D}}
\def\mbE{\mathbf{E}}
\def\mbF{\mathbf{F}}
\def\mbG{\mathbf{G}}
\def\mbH{\mathbf{H}}
\def\mbI{\mathbf{I}}
\def\mbJ{\mathbf{J}}
\def\mbK{\mathbf{K}}
\def\mbL{\mathbf{L}}
\def\mbM{\mathbf{M}}
\def\mbN{\mathbf{N}}
\def\mbO{\mathbf{O}}
\def\mbP{\mathbf{P}}
\def\mbQ{\mathbf{Q}}
\def\mbR{\mathbf{R}}
\def\mbS{\mathbf{S}}
\def\mbT{\mathbf{T}}
\def\mbU{\mathbf{U}}
\def\mbV{\mathbf{V}}
\def\mbW{\mathbf{W}}
\def\mbX{\mathbf{X}}
\def\mbY{\mathbf{Y}}
\def\mbZ{\mathbf{Z}}

% Caligraphy upper case English alphabets
\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calC{\mathcal{C}}
\def\calD{\mathcal{D}}
\def\calE{\mathcal{E}}
\def\calF{\mathcal{F}}
\def\calG{\mathcal{G}}
\def\calH{\mathcal{H}}
\def\calI{\mathcal{I}}
\def\calJ{\mathcal{J}}
\def\calK{\mathcal{K}}
\def\calL{\mathcal{L}}
\def\calM{\mathcal{M}}
\def\calN{\mathcal{N}}
\def\calO{\mathcal{O}}
\def\calP{\mathcal{P}}
\def\calQ{\mathcal{Q}}
\def\calR{\mathcal{R}}
\def\calS{\mathcal{S}}
\def\calT{\mathcal{T}}
\def\calU{\mathcal{U}}
\def\calV{\mathcal{V}}
\def\calW{\mathcal{W}}
\def\calX{\mathcal{X}}
\def\calY{\mathcal{Y}}
\def\calZ{\mathcal{Z}}

% Numbers
\def\bzero{\boldsymbol{0}}
\def\bone{\boldsymbol{1}}

% Sets and notations
\newcommand{\binaryB}[1]{\mathds{B}^{#1}}
\newcommand{\complexC}[1]{\mathds{C}^{#1}}
\newcommand{\expecE}[1]{\mathds{E}\left\{{#1}\right\}}
\newcommand{\naturalN}[1]{\mathds{N}^{#1}}
\newcommand{\probP}[1]{\mathds{P}\mathrm{r}\left\{{#1}\right\}}
\newcommand{\rationalQ}[1]{\mathds{Q}^{#1}}
\newcommand{\realR}[1]{\mathds{R}^{#1}}
\newcommand{\realRp}[1]{\mathds{R}_{+}^{#1}}
\newcommand{\realRn}[1]{\mathds{R}_{-}^{#1}}
\newcommand{\integerZ}[1]{\mathds{Z}^{#1}}

% Matrix terms
\def\tr#1{\mathrm{Tr}\left(#1\right)}
\def\vec#1{\mathrm{vec}\left(#1\right)}
\def\diag#1{\mathrm{diag}\left(#1\right)}
\def\Diag#1{\mathrm{Diag}\left(#1\right)}
\def\bdiag#1{\mathbf{diag}\left(#1\right)}
\def\cov#1{\mathrm{cov}\left(#1\right)}
\def\Cov#1{\mathrm{Cov}\left(#1\right)}
\def\bcov#1{\mathbf{cov}\left(#1\right)}

% Misc
\def\asin#1{\sin^{-1}\left(#1\right)}
\def\acos#1{\cos^{-1}\left(#1\right)}
\def\atan#1{\tan^{-1}\left(#1\right)}
\def\acsc#1{\csc^{-1}\left(#1\right)}
\def\asec#1{\sec^{-1}\left(#1\right)}
\def\acot#1{\cot^{-1}\left(#1\right)}
\def\implies{\Rightarrow}
\def\half{\frac{1}{2}}
\def\roothalf{\frac{1}{\sqrt{2}}}
\def\third{\frac{1}{3}}
\def\quarter{\frac{1}{4}}
\def\fourth{\frac{1}{4}}
\def\fifth{\frac{1}{5}}
\def\threequarter{\frac{3}{4}}
\def\ejomg{e^{j\omega}}
\def\ejnomg{e^{-j\omega}}
\def\zinv{z^{-1}}
\def\sgn#1{\mathrm{sgn}\left(#1\right)}
\def\sign#1{\mathrm{sign}\left(#1\right)}
\def\csign#1{\mathrm{csign}\left(#1\right)}
\def\deg{^\circ}
\def\Oh#1{\mathcal{O}\left(#1\right)}
\def\oh#1{o\left(#1\right)}
\def\d#1{\mathrm{d}#1}
\def\st{~\mathrm{s.t.}~}
\def\ow{~\mathrm{otherwise}~}
\def\ew{~\mathrm{elsewhere}~}
\def\eg{\emph{e.g.}}
\def\ie{\emph{i.e.}}
\def\wrt{\emph{w.r.t.~}}
\def\etal{\emph{et al.}}
\def\etc{\emph{etc.~}}
\def\viz{\emph{viz.}}
\def\conv{\circledast}

% Basic text colors
\def\white#1{\textcolor{white}{#1}}
\def\black#1{\textcolor{black}{#1}}
\def\red#1{\textcolor{red}{#1}}
\def\green#1{\textcolor{green}{#1}}
\def\blue#1{\textcolor{blue}{#1}}
\def\cyan#1{\textcolor{cyan}{#1}}
\def\magenta#1{\textcolor{magenta}{#1}}
\def\yellow#1{\textcolor{yellow}{#1}}

% Special colors that comes with [dvipsnames] option in xcolor package
\def\Apricot#1{\textcolor{Apricot}{#1}}
\def\Aquamarine#1{\textcolor{Aquamarine}{#1}}
\def\Bittersweet#1{\textcolor{Bittersweet}{#1}}
\def\Black#1{\textcolor{Black}{#1}}
\def\Blue#1{\textcolor{Blue}{#1}}
\def\BlueGreen#1{\textcolor{BlueGreen}{#1}}
\def\BlueViolet#1{\textcolor{BlueViolet}{#1}}
\def\BrickRed#1{\textcolor{BrickRed}{#1}}
\def\Brown#1{\textcolor{Brown}{#1}}
\def\BurntOrange#1{\textcolor{BurntOrange}{#1}}
\def\CadetBlue#1{\textcolor{CadetBlue}{#1}}
\def\CarnationPink#1{\textcolor{CarnationPink}{#1}}
\def\Cerulean#1{\textcolor{Cerulean}{#1}}
\def\CornflowerBlue#1{\textcolor{CornflowerBlue}{#1}}
\def\Cyan#1{\textcolor{Cyan}{#1}}
\def\Dandelion#1{\textcolor{Dandelion}{#1}}
\def\DarkOrchid#1{\textcolor{DarkOrchid}{#1}}
\def\Emerald#1{\textcolor{Emerald}{#1}}
\def\ForestGreen#1{\textcolor{ForestGreen}{#1}}
\def\Fuchsia#1{\textcolor{Fuchsia}{#1}}
\def\Goldenrod#1{\textcolor{Goldenrod}{#1}}
\def\Gray#1{\textcolor{Gray}{#1}}
\def\Green#1{\textcolor{Green}{#1}}
\def\GreenYellow#1{\textcolor{GreenYellow}{#1}}
\def\JungleGreen#1{\textcolor{JungleGreen}{#1}}
\def\Lavender#1{\textcolor{Lavender}{#1}}
\def\LimeGreen#1{\textcolor{LimeGreen}{#1}}
\def\Magenta#1{\textcolor{Magenta}{#1}}
\def\Mahogany#1{\textcolor{Mahogany}{#1}}
\def\Maroon#1{\textcolor{Maroon}{#1}}
\def\Melon#1{\textcolor{Melon}{#1}}
\def\MidnightBlue#1{\textcolor{MidnightBlue}{#1}}
\def\Mulberry#1{\textcolor{Mulberry}{#1}}
\def\NavyBlue#1{\textcolor{NavyBlue}{#1}}
\def\OliveGreen#1{\textcolor{OliveGreen}{#1}}
\def\Orange#1{\textcolor{Orange}{#1}}
\def\OrangeRed#1{\textcolor{OrangeRed}{#1}}
\def\Orchid#1{\textcolor{Orchid}{#1}}
\def\Peach#1{\textcolor{Peach}{#1}}
\def\Periwinkle#1{\textcolor{Periwinkle}{#1}}
\def\PineGreen#1{\textcolor{PineGreen}{#1}}
\def\Plum#1{\textcolor{Plum}{#1}}
\def\ProcessBlue#1{\textcolor{ProcessBlue}{#1}}
\def\Purple#1{\textcolor{Purple}{#1}}
\def\RawSienna#1{\textcolor{RawSienna}{#1}}
\def\Red#1{\textcolor{Red}{#1}}
\def\RedOrange#1{\textcolor{RedOrange}{#1}}
\def\RedViolet#1{\textcolor{RedViolet}{#1}}
\def\Rhodamine#1{\textcolor{Rhodamine}{#1}}
\def\RoyalBlue#1{\textcolor{RoyalBlue}{#1}}
\def\RoyalPurple#1{\textcolor{RoyalPurple}{#1}}
\def\RubineRed#1{\textcolor{RubineRed}{#1}}
\def\Salmon#1{\textcolor{Salmon}{#1}}
\def\SeaGreen#1{\textcolor{SeaGreen}{#1}}
\def\Sepia#1{\textcolor{Sepia}{#1}}
\def\YellowOrange#1{\textcolor{YellowOrange}{#1}}
\def\SkyBlue#1{\textcolor{SkyBlue}{#1}}
\def\SpringGreen#1{\textcolor{SpringGreen}{#1}}
\def\Tan#1{\textcolor{Tan}{#1}}
\def\TealBlue#1{\textcolor{TealBlue}{#1}}
\def\Thistle#1{\textcolor{Thistle}{#1}}
\def\Turquoise#1{\textcolor{Turquoise}{#1}}
\def\Violet#1{\textcolor{Violet}{#1}}
\def\VioletRed#1{\textcolor{VioletRed}{#1}}
\def\White#1{\textcolor{White}{#1}}
\def\WildStrawberry#1{\textcolor{WildStrawberry}{#1}}
\def\Yellow#1{\textcolor{Yellow}{#1}}
\def\YellowGreen#1{\textcolor{YellowGreen}{#1}}
\def\YellowOrange#1{\textcolor{YellowOrange}{#1}}

% Theorem-like environments (defs, lemmas numbered like Theorems)
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\declaretheorem[style=definition,name=Remark,qed=$\blacksquare$]{remark}

% algorithms
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Initialize:}}
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}
\algnewcommand\algorithmicinit{\textbf{Initialize:}}
\algnewcommand\Init{\item[\algorithmicinit]}
\def\Print#1{\textbf{print}~#1}
\def\To{\textbf{to}~}

% underbrace inside a matrix environment
\newcommand\undermat[2]{
	\makebox[0pt][l]{${\underbrace{\hphantom{
					\begin{matrix}#1\end{matrix}}}_{\text{$#2$}}}$}#1}
